Monte Carlo models of dust coagulation

The thesis deals with the first stage of planet formation, namely dust coagulation from micron to millimeter sizes in circumstellar disks. For the first time, we collect and compile the recent laboratory experiments on dust aggregates into a collision model that can be implemented into dust coagulation models. We put this model into a Monte Carlo code that uses representative particles to simulate dust evolution. Simulations are performed using three different disk models in a local box (0D) located at 1 AU distance from the central star. We find that the dust evolution does not follow the previously assumed growth-fragmentation cycle, but growth is halted by bouncing before the fragmentation regime is reached. We call this the bouncing barrier which is an additional obstacle during the already complex formation process of planetesimals. The absence of the growth-fragmentation cycle and the halted growth has two important consequences for planet formation. 1) It is observed that disk atmospheres are dusty throughout their lifetime. Previous models concluded that the small, continuously produced fragments can keep the disk atmospheres dusty. We however show that small fragments are not produced because bouncing prevents fragmentation. 2) As particles do not reach the fragmentation barrier, their sizes are smaller compared to the sizes reached in previous dust models. We decided to investigate point 1) in more detail. A vertical column of a disk (1D) is modeled including the sedimentation of the particles. We find that already intermediate levels of turbulence can prevent particles settling to the midplane.

==> Chapters/Chapter6.tex <==
% Chapter 6

\chapter{The first stages of planet formation in binary systems} % Write in your own chapter title
\label{chp:binary}
\lhead{Chapter 6. \emph{Planet formation in binary systems}} % Write in your own chapter title to set the page header
\rhead{}


